Looking Beyond Label Noise: Shifted Label Distribution Matters in Distantly Supervised Relation Extraction

In recent years there is a surge of interest in applying distant supervision (DS) to automatically generate training data for relation extraction (RE). In this paper, we study the problem what limits the performance of DS-trained neural models, conduct thorough analyses, and identify a factor that can influence the performance greatly, shifted label distribution. Specifically, we found this problem commonly exists in real-world DS datasets, and without special handing, typical DS-RE models cannot automatically adapt to this shift, thus achieving deteriorated performance. To further validate our intuition, we develop a simple yet effective adaptation method for DS-trained models, bias adjustment, which updates models learned over the source domain (i.e., DS training set) with a label distribution estimated on the target domain (i.e., test set). Experiments demonstrate that bias adjustment achieves consistent performance gains on DS-trained models, especially on neural models, with an up to 23% relative F1 improvement, which verifies our assumptions. Our code and data can be found at \url{https://github.com/INK-USC/shifted-label-distribution}.

==> 2exp_depricated.tex <==
% !TEX encoding = UTF-8
% !TEX Root = 0_main.tex

\section{Experiment Setup}

For a fair and meaningful comparison, we ensure the same experimental setup is applied in all experiments. 
Implementations will be made available online for future study.

\begin{table}[]
\footnotesize
\centering
\scalebox{0.9}{
\begin{tabularx}{1.1\columnwidth}{l*{3}{Y}}
\toprule
\multirow{2}{*}{Dataset} & \multicolumn{2}{c}{\textbf{\tiny Distantly Supervised}} & \multicolumn{1}{c}{\textbf{\tiny Human-annotated}} \\         & \multicolumn{1}{c}{KBP}  & \multicolumn{1}{c}{NYT}  & \multicolumn{1}{c}{TACRED} \\ \midrule
\#Relation Types  & 7        & 25     & 42          \\
\#Train Sentences & 23784    & 235982 & 37311     \\
\#Test Sentences  & 289      & 395    & 6277    \\ 
\bottomrule
\end{tabularx}
}
\caption{Statistics of Datasets Used in Our Study.}\label{tab-data}
\end{table}

\subsection{Problem Setting} 
Following the previous work~\cite{liu2017heterogeneous,ren2017cotype}, we conduct relation extraction at the \textit{sentence level}. 
Formally speaking, we refer the basic unit of relation relation as relation mention, 
% which is composed of one sentence and one ordered entity pair within the sentence. 
\ie, one sentence and one ordered entity pair within the sentence.
% The relation extraction task is to categorize each relation mention into a given set of relation types, or a Not-Target-Type (\textsc{None}). 
Then, the task is to categorize each relation mention into a given set of relation types, or a Not-Target-Type (\textsc{None}). 


\subsection{Datasets}
We conduct experiments on three popular relation extraction datasets.
Two of them are distantly supervised and one is human-annotated. Statistics of the datasets are summarized in Table \ref{tab-data}.

\noindent 
\textbf{KBP} \citep{ling2012fine} uses Wikipedia articles annotated with Freebase entries as the training set, and uses manually-annotated sentences from 2013 KBP slot filling assessment results \citep{ellis2012linguistic} as the test set.

\noindent 
\textbf{NYT} \citep{riedel2010modeling} contains New York Times news articles and has been heuristically annotated as the training set; and its test set is constructed manually \citep{hoffmann2011knowledge}.

\noindent 
\textbf{TACRED} \citep{zhang2017position} is a large-scale crowd-sourced dataset, and is sufficiently larger than other manually annotated datasets. 

\subsubsection{Pre-processing}

We leverage pre-trained GloVe \citep{pennington2014glove} embedding\footnote{\url{http://nlp.stanford.edu/data/glove.840B.300d.zip}}, and use the StanfordNLP toolkit~\citep{manning-EtAl:2014:P14-5} to get part-of-speech (POS) tags, named-entity recognition (NER) tags and dependency parsing trees.

As for the development set, we use the provided dev set on TACRED, and randomly split 10\% of training set as the dev set on KBP and NYT. \label{data-splitting}


\subsection{Relation Extraction Models}
We consider two popular classes of relation extraction models here, \ie, feature-based models and neural models. 
For each relation mention, most of these models will first construct a representation $\h$, and then make predictions based on $\h$. 
All models, except CoType-RM, adopt a softmax layer to make predictions:
\begin{equation}
p(y = r_i|\h) = \frac{\exp(\r_i^T\h + b_i)}{\sum_{r_j}\exp(\r_j^T\h+b_j)}
\label{eqn:softmax}
\end{equation}
where $\r_i$ and $b_i$ are the parameters corresponding to \textit{i}-th relation type. 

\input{table_1.tex}

\subsubsection{Feature-based Models}
%\qinyuan{add logistic regression}
We included three feature-based models, \ie, CoType-RM~\cite{ren2017cotype},  ReHession~\cite{liu2017heterogeneous}, and multi-class logistic regression.
For each relation mention $z$, these methods would first extract a list of features, $\F=\{f_1, f_2, ..., f_m\}$.
Detailed descriptions of these features are in Table~\ref{tbl:feature} Appendix~\ref{sec:appendix} .

\noindent \textbf{CoType-RM} 
is a variant of CoType~\citep{ren2017cotype}, a unified learning framework to get both the feature embedding and the label embedding. It leverages a partial-label loss to handle the label noise, and uses cosine similarity to conduct inference. 
Here, we only use its relation extraction part.

\noindent \textbf{ReHession} \citep{liu2017heterogeneous}
directly maps each feature to an embedding vector, 
treats their average as the relation mention representation $\h$, and uses a softmax to make predictions.
This method was initially proposed for heterogeneous supervision, and is modified to fit our distantly supervised RE task. 
Specifically, for a relation mention annotated with a set of relation $\Y=\{r_{l_1}, \cdots, r_{l_m}\}$, it would first calculate a cross entropy as the loss function:
\begin{equation}
\mathcal{L} = -\sum_{r_i} q(y=r_i |\Y, \h) \log p(y=r_i | \h)
\label{eqn:loss}
\end{equation}
where $p(.| \h)$ is defined in Equation~\ref{eqn:softmax}, and $q(.|\Y, \h)$ is used to encode supervision information in a self-adapted manner:
\begin{equation*}
q(y = r_i|\Y, \h) = \frac{\exp(\r_i^T\h+b_i) \cdot \mathbb{I}(r_i \in \Y) }{\sum_{r_j \in \Y}\exp(\r_j^T\h+b_j)}
\end{equation*}
We can find that when $|\Y| = 1$ (\ie only one label is assigned to the relation mention), $q(.|\Y, \h)$ would be one-hot and Equation~\ref{eqn:loss} becomes standard cross entropy loss. 

\noindent \textbf{Logistic Regression} is applied over the extracted features as a baseline method.\footnote{We use liblinear package from \url{https://github.com/cjlin1/liblinear}}

\subsubsection{Neural Models}
We employ several popular neural structures to calculate the sentence representation $\h$. As for the loss function, cross entropy as shown in Equation~\ref{eqn:loss} is used for all following neural models. 

\noindent \textbf{Bi-LSTMs and Bi-GRUs}
use two-layer bidirectional RNNs to encode sentences and concatenate their final states in the last layer as the representation~\cite{zhang2017position}. 
% Following previous work~\cite{zhang2017position}, we use two types of RNNs---Bi-LSTMs and Bi-GRUs. Both of them have 2 layers with 200d hidden state in each layer.

\noindent \textbf{PA-LSTM}
% \jun{Add its full name here to be consistent with 'For Position Aware LSTM' in 2.4}
computes sentence representation with an attention over the outputs of LSTM. 
It treats the last hidden state as the query and integrates a position encoding to calculate the attention~\citep{zhang2017position}.

\noindent \textbf{CNNs and PCNNs}
use convolution neural networks as the encoder. 
In particular, CNNs
% \jun{CNNS} 
directly appends max-pooling after the convolution layer~\cite{zeng2014relation};
PCNNs 
% \jun{PCNNS} 
uses entities to split each sentence into three pieces, and does max-pooling respectively on these three pieces after convolution. Their outputs are concatenated as the final output~\cite{zeng2015distant}.

\noindent \textbf{SDP-LSTM}
splits the shortest dependency path between entities into two sub-paths with their common ancestor node. Two sub-paths are fed into LSTM respectively, and two representations are concatenated as $\h$~\citep{xu2015classifying}.

\subsection{Training Details}
%We run each model for 5 times and report the average F1 score and standard deviation.

\noindent\textbf{Optimization.} 
We use Stochastic Gradient Descent (SGD) for all models.
Learning rate is set at 1.0 initially, and is dynamically updated during training. Once the loss on the dev set has no improvement for 3 consecutive epochs, the learning rate will be factored by 0.1.

\noindent\textbf{Hyper-parameters.}
For ReHession, dropout ~\citep{srivastava2014dropout} is applied on input features and after average pooling. We tried the two dropout rates in $\{0.0,0.1,0.2,0.3,0.4,0.5\}$.

% For Position Aware LSTM,
For PA-LSTM,
Bi-LSTM and Bi-GRU, dropout is applied at the input of the RNN, between RNN layers and after RNN layers. Following \cite{melis2017state} we tried input and output 
% dropout probability \jun{dropout rate}
dropout rate
in $\{0.4,0.5,0.6,0.7,0.8\}$, and intra-layer 
% dropout probability \jun{dropout rate} 
dropout rate
in $\{0.1,0.2,0.3,0.4\}$.
We consider them as three separate hyper-parameters and tune them greedily.
Following previous work \cite{zhang2017position}, dimension of hidden states are set at 200.

Following \citet{lin2016neural}, the number of kernels is set to 230 for CNNs and PCNNs, and the window size is set at 3. Dropout is applied after pooling and $\tanh$ activation . We tried the dropout rates in $\{0.1,0.2,0.3,0.4,0.5\}$.

% % \section{Experiment Settings}
% \section{Experiment Setup}

% For a fair and meaningful comparison, we ensure the same experimental setup in all experiments. All implementations will be available online.

% \begin{table}[]
% \footnotesize
% \centering
% \begin{tabular}{l|cc|c}
% \hline
% \multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{\textbf{\tiny Distantly Supervised}} & \multicolumn{1}{c}{\textbf{\tiny Human-annotated}} \\         & \multicolumn{1}{c}{KBP}  & \multicolumn{1}{c|}{NYT}  & \multicolumn{1}{c}{TACRED} \\ \hline\hline
% %Train             & Noisy    & Noisy  & Clean  & Clean   \\
% %Test              & Clean    & Clean  & Clean  & Clean   \\
% \#Relation Types  & 7        & 25     & 42          \\
% \#Train Sentences & 23784    & 235982 & 37311     \\
% \#Test Sentences  & 289      & 395    & 6277    \\ \hline
% \end{tabular}
% \caption{Statistics of Datasets Used in Our Study.}\label{tab-data}
% \end{table}

% \subsection{Problem Setting} 
% Following the previous work~\cite{liu2017heterogeneous,ren2017cotype}, we conduct relation extraction at \textit{sentence level}. 
% Formally speaking, the basic unit is the relation mention, which is composed of one sentence and one ordered entity pair within the sentence. 
% The relation extraction task is to categorize each relation mention into a given set of relation types, or a Not-Target-Type (\textsc{None}). 

% \subsection{Datasets}
% We select three popular relation extraction datasets as benchmarks. Two of them are distantly supervised and one is human-annotated. Statistics of the datasets are summarized in Table \ref{tab-data}.

% \noindent 
% \textbf{KBP} \citep{ling2012fine} uses Wikipedia articles annotated with Freebase entries as train set, and manually-annotated sentences from 2013 KBP slot filling assessment results \citep{ellis2012linguistic} as test set.

% \noindent 
% \textbf{NYT} \citep{riedel2010modeling} contains New York Times news articles and has been already heuristically annotated. 
% Test set is constructed manually \citep{hoffmann2011knowledge}.

% \noindent 
% \textbf{TACRED} \citep{zhang2017position}  is a large-scale crowd-sourced dataset, and is sufficiently larger than other manually annotated datasets. 

% \subsubsection{Pre-Processing}

% We leverage pre-trained GloVe \citep{pennington2014glove} embedding\footnote{\url{http://nlp.stanford.edu/data/glove.840B.300d.zip}}, and use the StanfordNLP toolkit~\citep{manning-EtAl:2014:P14-5} to get part-of-speech (POS) tags, named-entity recognition (NER) tags and dependency parsing trees.

% As for the development set, we use the provided dev set on TACRED, and randomly split 10\% of training set as dev set on KBP and NYT. \label{data-splitting}



% \subsection{Relation Extraction Models}
% We consider two popular classes of relation extraction models here, \ie, feature-based models and neural models. 
% For each relation mention, these models will first construct a representation $\h$, and then make predictions based on $\h$. 
% All models, except CoType-RM, adopt a softmax layer to make predictions:
% \begin{equation}
% p(y = r_i|\h) = \frac{\exp(\r_i^T\h + b_i)}{\sum_{r_j}\exp(\r_j^T\h+b_j)}
% \label{eqn:softmax}
% \end{equation}
% where $\r_i$ and $b_i$ are the parameters corresponding to \textit{i}-th relation type. 
% % Still, these models use different ways to construct $\h$. 

% % For feature-based models, we extract features from instances with manually selected templates, learn embeddings for text features, relation mentions and type labels, and infer relation with the learned embeddings. 
% % % how to summarize cotype?
% % For neural models, we use information such as word embedding, entity position, part-of-speech tag as input to learn a representation vector of the instance, and adopt classifier during inference.
% % % For neural models, we apply neural networks on the sentence and feed the representation vector of the sentence to a classifier. 

% % Please note that all models, except CoType-RM, adopt a softmax layer for classification as the last stage. We hereby denote the sentence representation created with previous stages as $\mathbf{h}$, the linear layer as $\mathbf{Wh}+\mathbf{b}$, and results after softmax normalization as $p(y|\mathbf{h})$. The $i$th row vector of $\mathbf{W}$, representing the $i$th relationship $y_i$, will be denoted with $\mathbf{w}_i$. These notations will be repeatedly used in later parts.

% \input{table_1.tex}

% \subsubsection{Feature-based Models}
% % (put the feature table from cotype paper here)

% % \noindent \textbf{Manually Selected Features}

% We included two recent feature-based models, \ie, ReHession~\cite{liu2017heterogeneous} and CoType~\cite{ren2017cotype}. 
% For each relation mention $z$, these two methods would first extract a list of features, $\F=\{f_1, f_2, ..., f_m\}$.
% % These features require additional resources like POS-tagging and brown clustering.
% %Some of the features require additional resources such as POS-tags and brown clustering.
% % We include a detailed description in Appendix~\ref{sec:appendix}.
% Detailed descriptions of these features are in Appendix~\ref{sec:appendix} Table~\ref{tbl:feature}.

% % Given sentence $d$ and entities $e_1$ and $e_2$, we follow the practice in \citep{ren2017cotype} and extract feature strings $\mathcal{F}=\{f_1, f_2, ..., f_m\}$ according to manually selected templates. Detailed description of the templates can be found in Appendix \ref{sec:appendix}.
% % %The selected features, including context n-grams, part-of-speech tags and brown clustering results, capture comprehensive information about the sentence and entities. 
% % %A summary for the features used is shown in table ... [todo]
% % %For example, string ``EM\_DISTANCE\_5'' is used to describe the number of tokens between two entity mentions. 

% % \noindent \textbf{Feed-forward Neural Network (FFNN)}
% % %This part on FFNN can be longer, if needed.
% % FFNN maps each feature string $f_i$ in $\mathcal{F}$ to a real-value feature vector $\mathbf{f}_i$, and employs average pooling for the feature vectors to create a sentence representation $\mathbf{h}$.
% % % \begin{equation}
% % %     \mathbf{h}=\frac{1}{|\mathcal{F}|}\sum_{i=1}^{|\mathcal{F}|}\mathbf{f}_i
% % % \end{equation}
% % The model then measures the conditional probability $p(y_i|\mathbf{h})$ of each relation candidate $y_i$ with a classifier.
% % %More specifically, each feature string $f$ is given an index, and mapped to a real-value feature vector $\mathbf{f}$. As the number of features for each sentence varies, we employ average pooling for the feature vectors extracted from one sentence. 
% % %A linear layer is applied to the sentence representation vector $\mathbf{s}$ followed by softmax layer for classification.
% % To prevent overfitting, dropout \citep{srivastava2014dropout} is used on input features and before the linear layer.
% % % \end{itemize}

% \noindent \textbf{CoType-RM} 
% is a variant of CoType~\citep{ren2017cotype}, a unified learning framework to get both the feature embedding and the label embedding. It leverages a partial-label loss to handle the label noise, and uses cosine similarity to conduct inference. 
% Here, we  
% % only keeps the relation extraction term $\mathcal{O}_Z$ in CoType's objective function.
% % only use its relation extraction loss for our task.
% only use its relation extraction part.
% %which drops the entity part $O_M$ and entity-relation joint part $O_{ZM}$ in CoType's objective function.

% \noindent \textbf{ReHession} \citep{liu2017heterogeneous}
% % FFNN maps each feature string $f_i$ in $\mathcal{F}$ to a real-value feature vector $\mathbf{f}_i$, and employs average pooling for the feature vectors to create a sentence representation $\mathbf{h}$.
% %  maps each feature string $f_i$ in $\mathcal{F}$ to a real-value feature vector $\mathbf{f}_i$, and employs average pooling for the feature vectors to create a sentence representation $\mathbf{h}$.
% % The model then measures the conditional probability $p(y_i|\mathbf{h})$ of each relation candidate $y_i$ with a classifier.
% % To prevent overfitting, dropout \citep{srivastava2014dropout} is used on input features and before the linear layer.
% directly maps each feature to an embedding vector, % use an average pooling to construct the relation mention representation from feature embedding. 
% treats their average as the relation mention representation, and uses a softmax to make predictions.
% This method was initially proposed for heterogeneous supervision, and is modified to fit our distantly supervised RE task. 
% Specifically, for a relation mention annotated with a set of relation $\Y=\{r_{l_1}, \cdots, r_{l_m}\}$, it would first calculate a cross entropy as the loss function:
% % $$
% \begin{equation}
% \mathcal{L} = -\sum_{r_i} q(y=r_i |\Y, \h) \log p(y=r_i | \h)
% \label{eqn:loss}
% \end{equation}
% where $p(.| \h)$ is defined in Equation~\ref{eqn:softmax}, and $q(.|\Y, \h)$ is used to encode supervision information in a self-adapted manner:
% \begin{equation*}
% q(y = r_i|\Y, \h) = \frac{\exp(\r_i^T\h+b_i) \cdot \mathbb{I}(r_i \in \Y) }{\sum_{r_j \in \Y}\exp(\r_j^T\h+b_j)}
% % \label{eqn:softmax}
% \end{equation*}
% We can find that when $|\Y| = 1$ (\ie only one label is assigned to the relation mention), $q(.|\Y, \h)$ would be one-hot and Equation~\ref{eqn:loss} becomes standard cross entropy loss. 

% \subsubsection{Neural Models}
% We employed several popular neural structure to calculate the sentence representation $\h$. As for the loss function, cross entropy as shown in Eq.~\ref{eqn:loss} is used for all following neural models. 

% \noindent \textbf{Bi-LSTMs and Bi-GRUs}
% use bidirectional RNNs to encode sentences and concatenate their final states in the last layer as the representation. 
% Following previous work~\cite{zhang2017position}, we use two types of RNNs---Bi-LSTMs and Bi-GRUs. Both of them have 2 layers with 200d hidden state in each layer.

% \noindent \textbf{PA-LSTM}
% computes sentence representation with an attention over the outputs of LSTMs. 
% It treats the last hidden state as the query and integrates a position encoding to calculate the attention~\citep{zhang2017position}.

% \noindent \textbf{CNN and PCNN}
% use convolution neural networks as the encoder. 
% In particular, CNN directly appends max-pooling after the convolution layer~\cite{zeng2014relation};
% PCNN uses entities to split each sentence into three pieces, and does max-pooling respectively on these three pieces after the convolution layer. Their outputs are concatenated as the final output~\cite{zeng2015distant}.

% \noindent \textbf{SDP-LSTM}
% splits the shortest dependency path between entities into two sub-paths with their common ancestor nodes. Two sub-paths are fed into LSTM respectively, and two representations are concatenated as $\h$~\citep{xu2015classifying}.

% \subsection{Training Details}
% We run each model for 5 times and report the average F1 and standard deviation.

% \noindent\textbf{Optimization.} 
% We use Stochastic Gradient Descent (SGD) for all models.
% Learning rate is set at 1.0 initially, and is dynamically updated during training. Once the loss on the dev set has no improvement for 3 consecutive epochs, the learning rate will be factored by 0.1.

% \noindent\textbf{Hyper-parameters.}
% For ReHession, dropout is applied on input features and after average pooling. We tried the two dropout rates in $\{0.0,0.1,0.2,0.3,0.4,0.5\}$.

% For Position Aware LSTM, Bi-LSTM and Bi-GRU, dropout \citep{srivastava2014dropout} is applied at the input of the RNN, between RNN layers and after RNN before linear layer. Following \cite{melis2017state} we tried input and output dropout probability in $\{0.4,0.5,0.6,0.7,0.8\}$, and intra-layer dropout probability in $\{0.1,0.2,0.3,0.4\}$.
% We consider them as three separate hyper-parameters and tune them greedily.
% Following previous work \cite{zhang2017position}, dimension of hidden states are set at 200.

% Following previous work~\cite{lin2016neural}, the number of kernels is set to 230 for CNN or PCNN, and the window size is set at 3. Dropout is applied after pooling and $\tanh$ activation . We tried the dropout rates in $\{0.1,0.2,0.3,0.4,0.5\}$.

==> fig_code/fig_shifted.tex <==
\begin{figure}
\centering
\begin{minipage}{.29\textwidth}
  \centering
  \includegraphics[trim={2.1cm, 1.2cm, 0.5cm, 1.5cm},clip,width=\linewidth]{figures/merge_distr2.pdf}
\end{minipage}%
\begin{minipage}{.21\textwidth}
  \centering
  \includegraphics[trim={0.1cm, 1.5cm, 0cm, 2.0cm},clip,width=\linewidth]{figures/merge_distr.pdf}
\end{minipage}
% \vspace{-0.25cm}
\caption{\textbf{Left:} Label distributions of KBP (distantly supervised dataset) are shifted, while those of TACRED (human-annotated dataset, 6 classes for illustration) are consistent. Full distributions for NYT and TACRED can be found in Appendix~\ref{sec:appendix}.
\textbf{Right:} Each relation $r_i$ is categorized into intervals along x-axis according to $\left|p(r_i|\mathcal{D}_{train})-p(r_i|\mathcal{D}_{test})\right|$; height of the bars indicates proportion of instances that fall into each category, revealing that the shift is severe in DS datasets such as KBP and NYT.}
\label{fig:shifted_distrib}
% \vspace{-0.5cm}
\end{figure}

==> old_0abs.tex <==
% !TEX encoding = UTF-8
% !TEX Root = 0_main.tex

\begin{abstract}
% In recent years, there is a surge of interest in developing distantly supervised methods for relation extraction. While extensive efforts have been spent on making models robust to label noise in training data, we observe that performance gain of state-of-the-art neural models (over simple feature-based models) diminishes when trained with distantly supervised data instead of human-annotated data--an observation that motivates our study on other hidden factors limiting model performance.

In recent years there is a surge of interest in applying distant supervision (DS) to automatically generate training data for relation extraction. However, despite extensive efforts have been done on constructing advanced neural models for relation extraction, our experiments reveal that these neural models demonstrate only similar (or even worse) performance as compared with simple feature-based methods on DS datasets.
%---in contrast, these neural models significantly outperform feature-based methods on human-annotated dataset.
% In this paper, going beyond label noise, we conduct thorough experimental studies to reveal an important yet long-overlooked issue in distantly-supervised relation extraction--\textit{shifted labeled distribution}. This issue is recognized during the analysis of two heuristic threshold techniques which are found to be effective on distantly supervised data but not on human-annotated data.
In this paper, we conduct thorough analysis to answer the question \textit{what other factors limit the performance of DS-trained neural models?} Experimental results show that \textit{shifted labeled distribution} commonly exists on real-world DS datasets, and impact of this issue is further validated on synthetic datasets.
%  for all models.
% Building upon this new insight, we conduct extensive experiments on synthetic datasets with different level of label distribution shift. Results of these experiments validate our hypothesis and emphasize the impact brought by such shift. We also introduce a principled adaptation method in evaluation---bias adjustment, which adjusts the model along the shift and achieves improved performance, again indicating the severity of this issue.
Building upon the new insight, we develop a simple yet effective adaptation method for DS methods, called \textit{bias adjustment}, to update models learned over source domain (\ie, DS training set) with label distribution estimated on target domain.
%using a small development set sampled from the target domain (i.e., original evaluation set).
Experiments demonstrate that bias adjustment achieves consistent performance gains on all methods, especially on neural models, with up to a 22\% relative F1 improvement.
%we further propose a principled model adaptation approach to explicitly deal with the shifted distribution, which can easily cope with existing relation extraction models. We observe consistent performance gains for all compared methods on multiple distant supervision datasets, with up to a 22\% relative F1 improvement.
\end{abstract}

% Version 1
% \begin{abstract}
% Effort-light relation extraction via distant supervision has been pursued for years. Going beyond label noise, we show extensive experimental analysis that underlies the recognition of a long-overlooked yet important issue -- shifted label distribution. In particular, we first discuss the inconsistent performance of neural models, \ie, noticeable improvements are made by these models on gold standard corpora but deceased remarkably with distant supervision. Further exploration leads us towards two heuristic techniques that can boost the performance a lot. Conjecturing their underlying mechanism to be a better handling of the shifted label distribution, we studied such shift and found it to be impactful. To explicitly tackle this problem, we further develop a simple and effective method to adapt models along the shift. This method can be easily augmented to popular models, and we observe consistent improvements for all compared methods on both distant supervised corpora, with a up to 13\% of relative F1 boost.
% \end{abstract}

% % Version 2
% \begin{abstract}
% Effort-light relation extraction via distant supervision has been pursued for years.
% Going beyond label noise, we show extensive experimental analysis that underlies the recognition of a long-overlooked yet important issue -- shifted label distribution. 
% In particular, we first discuss the inconsistent performance of neural models, \ie, noticeable improvements are made by these models on gold standard corpora but deceased remarkably with distant supervision. 
% Conjecturing their underlying mechanism to be the shifted label distribution, we studied such shift and found it to be impactful. 
% To explicitly tackle this problem, we further develop a simple and effective method to adapt models along the shift. 
% This method can be easily augmented to popular models, and we observe consistent improvements for all compared methods on both distant supervised corpora, with a up to 13\% of relative F1 boost.
% \end{abstract}


% \begin{abstract}
% % %In this paper, we aim to explain the inconsistent behavior of existing models on clean and noisy data with observation from strictly designed experiments. 
% % We report inconsistent results of existing relation extraction models on clean (annotated mannually) and noisy (annotated with distant supervision) data. 
% % State-of-the-art models designed for clean datasets only have results comparable with simple baselines on noisy datasets. 
% % We aim to explain this \textit{diminishing} phenomenon with strictly designed experiments.
% % We find that imbalanced distributions between train and test set is an important problem, which is often ignored in previous works. 
% % In light of this, techniques such as thresholding and bias term adjustement are adopted and thoroughly discussed. 
% % We also show that selective attention, a prevalent denoising method, has limited effects in sentence-level setting, and does not necessarily solve the distribution problem. 
% % We would like to address that fundamental bottlenecks such as distribution difference should also be taken seriously.
% % %has limited effects on sentence-level settng \textcolor{purple}{[to be verified]}, and 
 
% % Effort-light training via distant supervision has been pursued for years, and the fundamental challenge lies in the noisy nature of automatically generated labels. 
% % , and its fundamental challenge lies in the noisy nature of automatically generated labels. 
% Effort-light relation extraction via distant supervision has been pursued for years.
% % Conducting extensive experimental analysis, we recognize an important but long-overlooked issue,
% % With extensive experimental analysis, we recognize an important but long-overlooked issue,
% % In this paper, we show extensive experimental analysis that underlies the recognition of a long-overlooked yet important issue, 
% % Here we show extensive experimental analysis that underlies the recognition of a long-overlooked yet important issue, 
% % Here we show extensive experimental analysis that underlies the recognition of a long-overlooked yet important issue, 
% % halting outstanding performance, 
% % blocking outstanding performance
% Going beyond label noise, we show extensive experimental analysis that underlies the recognition of a long-overlooked yet important issue -- shifted label distribution. 
% % Inspired by the inconsistent performance of neural models, 
% % In particular, starting from analyzing popular relation extraction models, we observe the superiority 
% % with gold standard annotation, neural models brought remarkable improvements over feature based models; however, with distant supervision, it's hard to observe such superiority. 
% % In particular, starting from analyzing popular relation extraction models, we observe remarkable decline of neural models' superiority on distant supervision. 
% % In particular, starting from analyzing popular relation extraction models, we observe the superiority of neural models decline remarkable on distant supervision. 
% % In particular, we first observe the improvement of neural models decline remarkable on distant supervision. 
% % In particular, we first discuss the inconsistent performance of neural models, \ie, remarkable improvements are made by these models on gold standard corpora but deceased with distant supervision. 
% In particular, we first discuss the inconsistent performance of neural models, \ie, noticeable improvements are made by these models on gold standard corpora but deceased remarkably with distant supervision. 
% % Further exploration leads us towards two empirically technique that can boost the performance a lot.
% Further exploration leads us towards two heuristic techniques that can boost the performance a lot.
% % Conjecturing their underlying mechanism to be handling the shifted label distribution, we studied the impact of such shift, and found the results supporting our argument. 
% % Conjecturing their underlying mechanism to be a better handling of the shifted label distribution, we studied the impact of such shift, and found the results supporting our argument. 
% % Conjecturing their underlying mechanism to be a better handling of the shifted label distribution, we studied the impact of such shift, and the results reveal the importance of ....
% Conjecturing their underlying mechanism to be a better handling of the shifted label distribution, we studied such shift and found it to be impactful. 
% % We further develop an explicit domain adaption technique for this problem, and observed consistent performance improvement for all methods on all distant supervised corpora, with a up to 25\% of improvement on F1 score. 
% % We further develop a simple and effective method to explicitly conduct domain adaption and help models to be robust to the shift.
% To explicitly tackle this problem, we further develop a simple and effective method to adapt models along the shift. 
% % We observe consistent performance improvement for all methods on all distant supervised corpora, with a up to 13\% of relative improvement on F1 score. 
% % We observe consistent performance improvement for all compared methods on both distant supervised corpora, with a up to 13\% of relative F1 improvement.
% This method can be easily augmented to popular models, and we observe consistent improvements for all compared methods on both distant supervised corpora, with a up to 13\% of relative F1 boost.

% \end{abstract}


==> table_tacred.tex <==
\begin{table*}[htbp!]
\centering %\footnotesize
\scalebox{0.75}{
\begin{tabular}{llccccccccc}
\hline
Dataset  & Model  & Original       & Max-thres & $\Delta$  & Ent-thres & $\Delta$ & Set Bias & $\Delta$ & Fix Bias & $\Delta$ \\ \hline\hline
\multirow{3}{*}{TACRED} & ReHession & 58.06 & 57.97 $\pm$ 0.57 & -0.09 & 57.91 $\pm$ 0.52 & -0.15 & 58.59 $\pm$ 0.66 & 0.53 & 58.61 $\pm$ 0.99 & 0.55\\
    & Bi-GRU       & 65.38 & 65.29 $\pm$ 0.58 & 0.01 & 65.38 $\pm$ 0.60 & 0.10 &63.72 $\pm$ 0.64 & -1.56 & 64.70 $\pm$ 0.46 & -0.68\\
    & Bi-LSTM      & 62.74 & 62.95 $\pm$ 0.35 & 0.21 & 62.67 $\pm$ 0.29 & -0.07 & 62.73 $\pm$ 0.60 & -0.01 & 63.44 $\pm$ 0.54 & 0.70\\
	\hline
\end{tabular}
}
\caption{F1 score of RE Models on TACRED} 
\label{table-tacred}
\vspace{-0.2cm}
\end{table*}

